Theory of processes

The book gives a detailed exposition of basic concepts and results of a theory of processes. The presentation of theoretical concepts and results is accompanied with illustrations of their application to solving various problems of verification of processes. Along with well-known results there are presented author's results related to verification of processes with message passing, and there are given examples of an application of these results.

==> newmacr.TEX <==
\def\poko#1#2#3{$$\diagrw{#1&
\prightline{#2}\!\!\!\!\to\!\!\!\!\to&\!\!#3}$$}

\def\cko#1#2#3{$$\diagrw{#1&
\pright{#2}&#3}$$}


\def\prightline#1{
  \begin{picture}(20,8)
  \put (-5,2.5){\line(1,0){30}}
  \put (9,8){\makebox(1,1){$\scriptstyle #1$}}
  \end{picture} }


\def\pu#1#2{
\mbox{$\!\!\begin{picture}(0,0)
\put (-#1,-#2){\line(1,0){#1}}
\put (-#1,-#2){\line(0,1){#2}}
\put (#1,#2){\line(-1,0){#1}}
\put (#1,#2){\line(0,-1){#2}}
\put (-#1,#2){\line(1,0){#1}}
\put (-#1,#2){\line(0,-1){#2}}
\put (#1,-#2){\line(-1,0){#1}}
\put (#1,-#2){\line(0,1){#2}}
\end{picture}$}
}

\def\pcycle#1{
  \begin{picture}(20,8)
  \put (-5,10){\line(1,0){30}}
  \put (9,15){\makebox(1,1){$\scriptstyle #1$}}
  \put (25,-4){\vector(-1,0){30}}
  \put(25,3){\oval(14,14)[r]}
  \end{picture} }


\def\krug#1{
\begin{picture}(16,16)
\put(8,4){\oval(16,16)}
\put(8,4){\makebox(0,0)[c]{$#1$}}
\end{picture}}

\def\kruginit#1{
\begin{picture}(16,16)
\put(8,4){\oval(16,16)}
\put(8,4){\oval(18,18)}
\put(8,4){\makebox(0,0)[c]{$#1$}}
\end{picture}}


\def\ak{
  \begin{picture}(18,20)
  \put (-5,0){\vector(1,1){30}}
  \put (-5,0){\vector(1,-1){30}}
  \end{picture} }


\def\prightleft#1#2{
  \begin{picture}(20,0)
  \put (-5,2){\vector(1,0){30}}
  \put (9,7){\makebox(1,1){$\scriptstyle #1$}}
  \put (25,-2){\vector(-1,0){30}}
  \put (9,-7){\makebox(1,1){$\scriptstyle #2$}}
  \end{picture} }



\def\be#1{\begin{equation}\label{#1}}
\def\ee{\end{equation}}
\def\re#1{(\ref{#1})}

\def\bn{\begin{enumerate}}
\def\en{\end{enumerate}}
\def\bi{\begin{itemize}}
\def\ei{\end{itemize}}
\def\i{\item}


\def\l#1{\langle #1 \rangle}
%\def\l#1{U(#1)}
\def\okr#1{U(#1)}

\def\c#1{\left\{\begin{array}{lllll}#1\end{array}\right\}}
\def\d#1{\left[\begin{array}{lllll}#1\end{array}\right]}
\def\b#1{\left(\begin{array}{lllll}#1\end{array}\right)}
\def\ra#1{\;\mathop{\to}\limits^{#1}\;}
\def\leqd{\;\mathop{<}\limits_{2}\;}

\def\by{\begin{array}{llllllllllllll}}
\def\ey{\end{array}}
\def\been{\begin{itemize}}
\def\enen{\end{itemize}}
\def\beenum{\begin{enumerate}}
\def\enenum{\end{enumerate}}
\def\eam{\mathbin{{\mathop{=}\limits^{\mbox{\scriptsize def}}}}}


\def\n{\par}
\def\v{{$\,\,\,\,\,$}}
\def\tostar{\mathbin{\to\!\!\!^*}}
\def\lrstar{\mathbin{\leftrightarrow\!\!\!^*}}
\def\tow#1{\mathbin{{\mathop{\to}\limits^{#1}}}}
\def\towstar#1{\mathbin{{\mathop{\to}\limits^{#1}\!\!^*}}}
\def\lrw#1{\mathbin{\mathop{\leftrightarrow}\limits^{#1}}}
\def\lrwstar#1{\mathbin{\mathop{\longleftrightarrow}
\limits^{#1}\!\!^*}}
\def\sep{{\,|\,}}
\def\Exists{{\exists\,}}
\def\beenum{\begin{enumerate}}
\def\enenum{\end{enumerate}}
\def\ba{\left\{\begin{array}{llllllllll}}
\def\ea{\end{array} \right\}}
\def\bau{\left[\begin{array}{llllllllll}}
\def\eau{\end{array} \right]}
\def\beq{\begin{equation}}


\def\pdownup#1{
  \begin{picture}(8,28)
  \put (1,24){\line(0,-1){28}}
  \put (7,-4){\vector(0,1){28}}
  \put(4,-4){\oval(6,6)[b]}
  \put (12,6){\makebox(1,1)[l]{$\scriptstyle #1$}}
  \end{picture} }



\def\pdown#1{
  \begin{picture}(8,28)
  \put (4,24){\vector(0,-1){31}}
  \put (7,6){\makebox(1,1)[l]{$\scriptstyle #1$}}
  \end{picture} }



\def\Rulesk#1#2{{\displaystyle\frac{\displaystyle #1}%
{\displaystyle #2}}}


\newenvironment{lettereq}[1]%
{\bgroup%
\def\theequation{$F_{\mbox{\scriptsize\arabic{equation}}}$}%
\setcounter{equation}{#1}%
\begin{eqnarray}}{\end{eqnarray}\egroup}

\def\blackbox{\vrule height 7pt width 7pt depth 0pt}

\def\bigblackbox{\vrule height 5557pt width 5557pt depth 0pt}


\def\teo#1{$\,$\\{\bf Theorem #1}\nopagebreak}

\def\lem#1{$\,$\\{\bf Lemma #1}\nopagebreak}

\def\sta#1{$\,$\\{\bf Statement #1}\nopagebreak}

\def\pro{$\,$\\{\bf Proof:}\nopagebreak}

\def\bo{\nopagebreak $\blackbox$\\}



\def\a#1{\mbox{$#1$}}

\def\ad{{\bf Ad\'amek J.}}

\def\app#1{\mathop{\approx}\limits_{#1}}

\def\App#1{\mathop{\approx}\limits_{#1}}

\def\bcd#1{
  \begin{picture}(20,20)
   \put(10,10){\circle{20}}
   \put(10,10){\mbox{#1}}
  \end{picture} }

\def\bcoam#1#2#3#4{
  \begin{picture}(20,20)
  \put (15,23){\vector(1,-3){20}}
  \put (15,-5){ \makebox(1,1)[r]{$\scriptstyle #1$}}
  \multiput (20,25)(3,-3){4}{\vector(1,-1){2}}
  \put(32,13){\vector(1,-1){3}}
  \put (27,19){\makebox(1,1)[l]{$\scriptstyle #2$}}
  \put (83,23){\vector(1,-3){20}}
  \put (85,-5){ \makebox(1,1)[r]{$\scriptstyle #4$}}
  \put (90,23){\vector(1,-1){15}}
  \put (95,18){ \makebox(1,1)[l]{$\scriptstyle #3$}}
  \end{picture} } 

\def\been{\begin{enumerate}}

\def\beit{\begin{itemize}}

\def\blackbox{\vrule height 7pt width 7pt depth 0pt}

\def\bm#1{\mathop{\leftrightarrow}\limits_{#1}}

\def\ci#1{$(#1)$ }

\def\cii#1{$(#1)$}

\def\cirsc{{\scriptscriptstyle\circ}}

\def\ciz#1{$(#1)$}

\def\corog#1#2#3{             \begin{picture}(20,20)
  \put (-35,23){\vector(3,-1){60}}
  \put (-8,8){\makebox(1,1)[r]{$\scriptstyle #1$}}
  \multiput (14,21)(3,-3){4}{\vector(1,-1){2}}
  \put (26,9){\vector(1,-1){3}}
  \put (22,17){\makebox(1,1)[l]{$\scriptstyle #2$}}
  \put (14,65){\vector(1,-3){19}}
  \put (24,40){\makebox(1,1)[l]{$\scriptstyle #3$}}
\end{picture} }
  
\def\db#1#2#3{[\![{#1},{#2}]\!]_{#3}}

\def\ddashright#1{
  \begin{picture}(20,8)
  \multiput (-5,3)(5,0){5}{\line(1,0){3}}
  \multiput (-5,0)(5,0){5}{\line(1,0){3}}
  \put (25,2){\line(-2,1){4}}
  \put (25,2){\line(-2,-1){4}}
  \put (9,7){\makebox(1,1){$\scriptstyle #1$}}
  \end{picture} }

\def\ddright#1{
  \begin{picture}(20,8)
  \put (-5,3){\line(1,0){28}}
  \put (-5,1){\line(1,0){28}}
  \put (25,2){\line(-2,1){4}}
  \put (25,2){\line(-2,-1){4}}
  \put (9,8){\makebox(1,1){$\scriptstyle #1$}}
  \end{picture} }

\def\diagr#1#2{\begin{equation}\label{#1}{
  \def\normalbaselines{\baselineskip20pt \lineskip3pt \lineskiplimit3pt }
  \matrix{#2}}\end{equation} }


\def\diagrw#1{{
  \def\normalbaselines{\baselineskip20pt \lineskip3pt \lineskiplimit3pt }
  \matrix{#1}}}


\def\rdiagr#1{$${
  \def\normalbaselines{\baselineskip20pt \lineskip3pt \lineskiplimit3pt }
  \matrix{#1}}$$ }


\def\dpright#1#2{    \begin{picture}(20,8)
    \put (-5,4){\vector(1,0){30}}
    \put (9,8){\makebox(1,1){$\scriptstyle #1$}}
    \put (-5,1){\vector(1,0){30}}
    \put (9,-3){\makebox(1,1){$\scriptstyle #2$}}
    \end{picture} }

\def\ddright#1{
  \begin{picture}(20,8)
  \put (-5,3){\line(1,0){28}}
  \put (-5,1){\line(1,0){28}}
  \put (25,2){\line(-2,1){4}}
  \put (25,2){\line(-2,-1){4}}
  \put (9,8){\makebox(1,1){$\scriptstyle #1$}}
  \end{picture} }

\def\eam{\buildrel \rm def \over =}
\def\eamxi{\buildrel \rm def \;\xi \over =}
\def\eamis{\buildrel \rm def \;I_s \over =}


\def\enen{\end{enumerate}}

\def\enit{\end{itemize}}

\def\ep{\;\mbox{$\mathop{\to}{\!\!\!\!\!.}$}\;}

\def\epi{\mbox{$\mathop{\to}\!\!\!\!\!\!\mathop{\to}$}}

\def\eqd{\buildrel \rm def \over\Longleftrightarrow}

\def\eqo{\mathop{\sim}\limits^o}

\def\exp#1#2#3#4{
\diagr{#3&\!\!\!\!\times\!\!\!\!&#1\cr
\pdashdownl{\hat{#4}}&\!\!\!\!
\begin{picture}(1,10)
\put (-3,3){\mbox{$\mathop{\times}$}}
\end{picture}\!\!\!\!
&\pdownr{id_#1}&\psearr{#4}\cr
#2^#1&\!\!\!\!\times\!\!\!\!&#1&\prightd{ev_{#1,#2}}&#2\cr
}}

\def\fd{${\cal F}_{\Phi,D}$}

\def\fuup#1#2{\mathop{#1}\limits^{#2}}

\def\goa{\mbox{$\Gamma$-$\Omega$-$Alg$ }}

\def\gs{\mbox{$\Gamma$-$Set$ }}

\def\hs#1{$(#1;[\![,]\!]_{#1})$}


\def\md{{\cal M}_D}

\def\mdn#1{{\cal M}_{D_#1}}

\def\mil#1{
\begin{picture}(20,20)
\put (30,3){\line(-1,0){5}}
\put (25,-7){\oval(20,20)[tl]}
\put (15,-7){\line(0,-1){71}}
\put (25,-78){\oval(20,20)[bl]}
\put (25,-88){\vector(1,0){5}}
\put (-2,-45){\makebox (16,8)[r]{$\scriptstyle #1$}}
\end{picture} }

\def\milcc#1{
\begin{picture}(20,20)
\put (33,3){\line(-1,0){2}}
\put (31,1){\oval(4,4)[tl]}
\put (29,1){\line(0,-1){74}}
\put (29,-73){\vector(1,-1){10}}
\put (9,-23){\makebox (16,8)[r]{$\scriptstyle #1$}}
\end{picture}}

\def\milongl#1{
\begin{picture}(20,20)
\put (30,3){\line(-1,0){5}}
\put (25,-7){\oval(20,20)[tl]}
\put (15,-7){\line(0,-1){115}}
\put (25,-122){\oval(20,20)[bl]}
\put (25,-132){\vector(1,0){5}}
\put (-2,-67){\makebox (16,8)[r]{$\scriptstyle #1$}}
\end{picture} }

\def\milongr#1{
\begin{picture}(20,20)
\put (-10,3){\line(1,0){5}}
\put (-5,-7){\oval(20,20)[tr]}
\put (5,-7){\line(0,-1){115}}
\put (-5,-122){\oval(20,20)[br]}
\put (-5,-132){\vector(-1,0){5}}
\put (8,-67){\makebox (16,8)[l]{$\scriptstyle #1$}}
\end{picture} }

\def\mir#1{
\begin{picture}(20,20)
\put (-10,3){\line(1,0){5}}
\put (-5,-7){\oval(20,20)[tr]}
\put (5,-7){\line(0,-1){71}}
\put (-5,-78){\oval(20,20)[br]}
\put (-5,-88){\vector(-1,0){5}}
\put (8,-45){\makebox (16,8)[l]{$\scriptstyle #1$}}
\end{picture} }

\def\mircc#1{
\begin{picture}(20,20)
\put (-10,3){\line(1,0){2}}
\put (-8,1){\oval(4,4)[tr]}
\put (-6,1){\line(0,-1){74}}
\put (-6,-73){\vector(-1,-1){10}}
\put (-10,-23){\makebox (1,8)[r]{$\scriptstyle #1$}}
\end{picture} }

\def\mironov#1{
\begin{picture}(20,20)
\put (-5,3){\line(1,0){45}}
\put (40,-7){\oval(20,20)[tr]}
\put (50,-7){\line(0,-1){68}}
\put (40,-75){\oval(20,20)[br]}
\put (40,-85){\vector(-1,0){45}}
\put (52,-40){\makebox (16,8){$\scriptstyle #1$}}
\end{picture} }

\def\mit#1{
\begin{picture}(20,20)
\put (10,-10){\line(0,1){5}}
\put (20,-5){\oval(20,20)[tl]}
\put (20,5){\line(1,0){100}}
\put (120,-5){\oval(20,20)[tr]}
\put (130,-5){\vector(0,-1){5}}
\put (-45,-2){\makebox (16,8)[r]{$\scriptstyle #1$}}
\end{picture} }

\def\mitblong#1{
\begin{picture}(20,20)
\put (10,15){\line(0,1){5}}
\put (20,15){\oval(20,20)[bl]}
\put (20,5){\line(1,0){225}}
\put (245,15){\oval(20,20)[br]}
\put (255,15){\vector(0,1){5}}
\put (138,10){\makebox (1,1)[c]{$\scriptstyle #1$}}
\end{picture} }

\def\mittlong#1{
\begin{picture}(20,20)
\put (10,-10){\line(0,1){5}}
\put (20,-5){\oval(20,20)[tl]}
\put (20,5){\line(1,0){225}}
\put (245,-5){\oval(20,20)[tr]}
\put (255,-5){\vector(0,-1){5}}
\put (138,10){\makebox (1,1)[c]{$\scriptstyle #1$}}
\end{picture} }

\def\ms#1#2{\{#1\;\vert\;#2\}}

\def\nr#1{\mathop{\preceq}\limits_{#1}}

\def\nro{\mathop{\preceq}}

\def\nrt{\mathop{\simeq}}

\def\oa{\mbox{$\Omega$-$Alg$ }}

\def\oc{\mathop{\approx}\limits^{+}}

\def\op#1#2{\langle{#1},{#2}\rangle}

%\def\oplus{\mathop{=}\limits^{+}}

\def\os{\mbox{$\Omega$-$Set$ }}

\def\pairarr#1#2{
\begin{picture}(10,10)
\put (0,6){$\mathop{\longrightarrow}$}
\put (6,11){\framebox(1,1){$\scriptstyle #1$}}
\put (0,4){$\mathop{\longleftarrow}$}
\put (6,2) {\framebox(1,1){$\scriptstyle #2$}}
\end{picture}}

\def\pbigbigright#1{
  \begin{picture}(50,8)
  \put (-15,3){\vector(1,0){80}}
  \put (24,8){\makebox(1,1){$\scriptstyle #1$}}
  \end{picture}}

\def\pbigdashright#1{
  \begin{picture}(50,8)
  \multiput (-20,3)(5,0){16}{\line(1,0){3}}
  \put (60,3){\vector(1,0){5}}
  \put (20,7){\makebox(1,1){$\scriptstyle #1$}}
  \end{picture} }

\def\pbigdownl#1{
  \begin{picture}(8,20)
  \put (4,20){\vector(0,-1){38}}
  \put (1-30){\makebox(1,1)[r]{$\scriptstyle #1$}}
  \end{picture} }

\def\pbigdownr#1{
  \begin{picture}(8,20)
  \put (4,20){\vector(0,-1){38}}
  \put (7,-30){\makebox(1,1)[l]{$\scriptstyle #1$}}
  \end{picture} }

\def\pbigright#1{
  \begin{picture}(50,8)
  \put (-5,3){\vector(1,0){60}}
  \put (24,8){\makebox(1,1){$\scriptstyle #1$}}
  \end{picture}}

\def\pdashdownl#1{
  \begin{picture}(8,20)
  \multiput (4,20)(0,-5){5}{\line(0,-1){3}}
  \put(4,-5){\vector(0,-1){5}}
  \put (1,6){\makebox(1,1)[r]{$\scriptstyle #1$}}
  \end{picture} }

\def\pdashdownr#1{
  \begin{picture}(8,20)
  \multiput (4,20)(0,-5){5}{\line(0,-1){3}}
  \put(4,-5){\vector(0,-1){5}}
  \put (7,6){\makebox(1,1)[l]{$\scriptstyle #1$}}
  \end{picture} }

\def\pdashmonoright#1{
  \begin{picture}(20,8)
  \multiput(-4,2)(5,0){5}{\line(1,0){3}}
  \put (21,2){\vector(1,0){5}}
  \put (-4,4){\oval(4,4)[l]}
  \put (-4,6){\line(1,0){2}}
  \put (11,6){\makebox(1,1){$\scriptstyle #1$}}
  \end{picture} }

\def\pdashnearr#1{
  \begin{picture}
  \put(-5,-10){\line(1,1){10}}
  \put(7,2){\line(1,1){10}}
  \put(19,14){\vector(1,1){10}}
  \put(10,5){\makebox(1,1)[l]{$\scriptstyle #1$}} 
  \end{picture} }

\def\pdashright#1{
  \begin{picture}(20,8)
  \multiput (-5,3)(5,0){5}{\line(1,0){3}}
  \put (20,3){\vector(1,0){5}}
  \put (9,7){\makebox(1,1){$\scriptstyle #1$}}
  \end{picture} }

\def\pdashsearl#1{
  \begin{picture}(20,20)
  \put (-5,20){\line (1,-1){10}}
  \put (7,8){\line (1,-1){10}}
  \put (19,-4){\vector(1,-1){10}}
  \put (-20,0){ \makebox(1,1)[r]{$\scriptstyle #1$}}
  \end{picture} }

\def\pdashsearr#1{
  \begin{picture}(20,20)
  \put (-5,20){\line (1,-1){10}}
  \put (7,8){\line (1,-1){10}}
  \put (19,-4){\vector(1,-1){10}}
    \put (12,5){\makebox(1,1)[l]{$\scriptstyle #1$}}
  \end{picture} }

\def\pdashswarl#1{
  \begin{picture}(20,20)
  \put (25,20){\vector(-1,-1){30}}
  \put (-15,5){\makebox(1,1)[r]{$\scriptstyle #1$}}
  \end{picture} }

\def\pdashswarr#1{
  \begin{picture}(20,20)
  \put (25,20){\vector(-1,-1){30}}
  \put (17,0){\makebox(1,1)[l]{$\scriptstyle #1$}}
  \end{picture} }

\def\pdoubledown#1#2{
\begin{picture}(8,20)
  \put (1,20){\vector(0,-1){30}}
  \put (-2,6){\makebox(1,1)[r]{$\scriptstyle #1$}}
  \put (5,20){\vector(0,-1){30}}
  \put (8,6){\makebox(1,1)[l]{$\scriptstyle #2$}}
  \end{picture}}

\def\pdownl#1{
  \begin{picture}(8,20)
  \put (4,20){\vector(0,-1){30}}
  \put (1,6){\makebox(1,1)[r]{$\scriptstyle #1$}}
  \end{picture} }

\def\pdownlongl#1{
  \begin{picture}(8,20)
  \put (4,20){\vector(0,-1){75}}
  \put (1,-16){\makebox(1,1)[r]{$\scriptstyle #1$}}
  \end{picture} }

\def\pdownlongr#1{
  \begin{picture}(8,20)
  \put (4,20){\vector(0,-1){75}}
  \put (7,-16){\makebox(1,1)[l]{$\scriptstyle #1$}}
  \end{picture} }

\def\pdownr#1{
  \begin{picture}(8,20)
  \put (4,20){\vector(0,-1){30}}
  \put (7,6){\makebox(1,1)[l]{$\scriptstyle #1$}}
  \end{picture} }

\def\pepidownl#1{
  \begin{picture}(8,20)
  \put (4,20){\vector(0,-1){30}}
  \put (4,-3){\vector(0,-1){5}}
  \put (1,6){\makebox(1,1)[r]{$\scriptstyle #1$}}
  \end{picture} }
  
\def\pepidownr#1{
  \begin{picture}(8,20)
  \put (4,20){\vector(0,-1){30}}
  \put (4,-3){\vector(0,-1){5}}
  \put (7,6){\makebox(1,1)[l]{$\scriptstyle #1$}}
  \end{picture} }

\def\pepiright#1{
  \begin{picture}(20,8)
  \put (-5,3){\vector(1,0){30}}
  \put (18,3){\vector(1,0){5}}
  \put (9,7){\makebox(1,1){$\scriptstyle #1$}}
  \end{picture} }

\def\pleftdouble#1#2
{
\begin{picture}(20,8)
  \put (25,5){\vector(-1,0){30}}
  \put (11,9){\makebox(1,1){$\scriptstyle {#1}$}}
  \put (25,1){\vector(-1,0){30}}
  \put (11,-3){\makebox(1,1){$\scriptstyle {#2}$}}
  \end{picture}
}

\def\plongright#1{
  \begin{picture}(20,8)
  \put (-5,3){\vector(1,0){115}}
  \put (50,8){\makebox(1,1){$\scriptstyle #1$}}
  \end{picture} }

\def\pmiddleright#1{
  \begin{picture}(35,8)
  \put (-5,3){\vector(1,0){45}}
  \put (17,8){\makebox(1,1){$\scriptstyle #1$}}
  \end{picture} }

\def\pmonodownl#1{
  \begin{picture}(8,20)
  \put (4,18){\vector(0,-1){28}}
  \put (6,18){\oval(4,4)[t]}
  \put (8,18){\line(0,-1){2}}
  \put (1,6){\makebox(1,1)[r]{$\scriptstyle #1$}}
  \end{picture} }
  
\def\pmonodownr#1{
  \begin{picture}(8,20)
  \put (4,18){\vector(0,-1){28}}
  \put (2,18){\oval(4,4)[t]}
  \put (0,18){\line(0,-1){2}}
  \put (7,6){\makebox(1,1)[l]{$\scriptstyle #1$}}
  \end{picture} }

\def\pmonoright#1{
  \begin{picture}(20,8)
  \put (-4,2){\vector(1,0){31}}
  \put (-4,4){\oval(4,4)[l]}
  \put (-4,6){\line(1,0){2}}
  \put (11,6){\makebox(1,1){$\scriptstyle #1$}}
  \end{picture} }

\def\pmonorighthigh#1{
  \begin{picture}(20,8)
  \put (-4,2){\vector(1,0){31}}
  \put (-4,4){\oval(4,4)[l]}
  \put (-4,6){\line(1,0){2}}
  \put (11,12){\makebox(1,1){$\scriptstyle #1$}}
  \end{picture} }

\def\pmonorightlong#1{
  \begin{picture}(20,8)
  \put (-9,2){\vector(1,0){41}}
  \put (-9,4){\oval(4,4)[l]}
  \put (-9,6){\line(1,0){2}}
  \put (11,6){\makebox(1,1){$\scriptstyle #1$}}
  \end{picture} }

\def\pnearr#1{
  \begin{picture}(20,20)
  \put (-5,-10){\vector(1,1){30}}
  \put (10,5){ \makebox(1,1)[l]{$\scriptstyle #1$}}
  \end{picture} }

\def\pneearr#1{
\begin{picture}(20,20)
  \put (0,0){\vector(3,2){40}}
  \put (1,2){ \makebox(1,1)[r]{$\scriptstyle #1$}}
  \end{picture}
}

\def\pnnearr#1{
  \begin{picture}(20,20)
  \put (-11,-10){\vector(1,2){38}}
  \put (10,28){ \makebox(1,1)[l]{$\scriptstyle #1$}}
  \end{picture} }

\def\pright#1{
  \begin{picture}(20,8)
  \put (-5,3){\vector(1,0){30}}
  \put (9,8){\makebox(1,1){$\scriptstyle #1$}}
  \end{picture} }


\def\prightdve#1{
  \begin{picture}(20,8)
  \put (-5,3){\vector(1,0){30}}
  \put (-2,3){\vector(1,0){30}}
  \put (9,8){\makebox(1,1){$\scriptstyle #1$}}
  \end{picture} }

\def\pleft#1{
  \begin{picture}(20,8)
  \put (25,3){\vector(-1,0){30}}
  \put (9,8){\makebox(1,1){$\scriptstyle #1$}}
  \end{picture} }

\def\prightd#1{
  \begin{picture}(20,8)
  \put (-5,3){\vector(1,0){30}}
  \put (9,-2){\makebox(1,1){$\scriptstyle #1$}}
  \end{picture} }

\def\prightdouble#1#2
{
\begin{picture}(20,8)
  \put (-5,5){\vector(1,0){30}}
  \put (11,10){\makebox(1,1){$\scriptstyle {#1}$}}
  \put (-5,1){\vector(1,0){30}}
  \put (11,-5){\makebox(1,1){$\scriptstyle {#2}$}}
  \end{picture}
}

\def\prightlong#1{
  \begin{picture}(20,8)
  \put (-5,3){\vector(1,0){35}}
  \put (11,7){\makebox(1,1){$\scriptstyle #1$}}
  \end{picture} }

\def\prightmiddle#1{
  \begin{picture}(20,8)
  \put (-10,3){\vector(1,0){40}}
  \put (9,8){\makebox(1,1){$\scriptstyle #1$}}
  \end{picture} }

\def\prightright#1{
  \begin{picture}(20,8)
  \put (-5,3){\vector(1,0){40}}
  \put (14,8){\makebox(1,1){$\scriptstyle #1$}}
  \end{picture} }

\def\prightsuperlong#1{
  \begin{picture}(20,8)
  \put (-5,3){\vector(1,0){49}}
  \put (18,7){\makebox(1,1){$\scriptstyle #1$}}
  \end{picture} }

\def\pseardouble#1{
  \begin{picture}(20,20)
  \put (-5,20){\vector(1,-1){30}}
  \put (-8,17){\vector(1,-1){30}}
  \put (1,2){ \makebox(1,1)[r]{$\scriptstyle #1$}}
  \end{picture} }

\def\psearl#1{
  \begin{picture}(20,20)
  \put (-5,20){\vector(1,-1){30}}
  \put (4,2){ \makebox(1,1)[r]{$\scriptstyle #1$}}
  \end{picture} }

\def\psearlongl#1{
  \begin{picture}(20,20)
  \put (-5,20){\vector(3,-1){105}}
  \put (41,-1){ \makebox(1,1)[r]{$\scriptstyle #1$}}
  \end{picture}}

\def\psearr#1{
  \begin{picture}(20,20)
  \put (-5,20){\vector(1,-1){30}}
    \put (10,8){\makebox(1,1)[l]{$\scriptstyle #1$}}
  \end{picture} }

\def\pnwarr#1{
  \begin{picture}(20,20)
  \put (25,-5){\vector(-1,1){30}}
	\put (14,10){\makebox(1,1)[l]{$\scriptstyle #1$}}
  \end{picture} }


\def\pseearl#1{
  \begin{picture}(20,20)
  \put (-20,40){\vector(3,-1){100}}
  \put (1,2){ \makebox(1,1)[r]{$\scriptstyle #1$}}
  \end{picture} }

\def\pseearr#1{
\begin{picture}(20,20)
  \put (-5,0){\vector(3,-2){40}}
  \put (1,2){ \makebox(1,1)[r]{$\scriptstyle #1$}}
  \end{picture}
}

\def\psesp#1{
  \begin{picture}(20,20)
  \put (15,20){\vector(2,-3){50}}
  \put (10,-25){ \makebox(22,8)[r]{$\scriptstyle #1$}}
  \end{picture} }

\def\psseardashr#1{
 \begin{picture}(20,20)
  \multiput(-5,20)(5,-10){5}{\line(1,-2){4}}
  \put (20,-30){\vector(1,-2){5}}
  \put (1,2){ \makebox(1,1)[r]{$\scriptstyle #1$}}
  \end{picture} }

\def\psseardouble#1#2{
  \begin{picture}(20,20)
  \put (-18,18){\vector(1,-1){70}}
  \put (-21,15){\vector(1,-1){70}}
  \put (3,-19){ \makebox(1,1)[r]{$\scriptstyle #1$}}
  \put (15,-13){ \makebox(1,1)[l]{$\scriptstyle #2$}}
  \end{picture} }

\def\pssearr#1
{
\begin{picture}(20,20)
  \put (-8,20){\vector(1,-2){37}}
  \put (10,-10){\makebox(1,1)[l]{$\scriptstyle {#1}$}}
\end{picture}
}

\def\pswarl#1{
  \begin{picture}(20,20)
  \put (25,20){\vector(-1,-1){30}}
  \put (9,8){\makebox(1,1)[r]{$\scriptstyle #1$}}
  \end{picture} }

\def\pswarr#1{
  \begin{picture}(20,20)
  \put (25,20){\vector(-1,-1){30}}
  \put (14,4){\makebox(1,1)[l]{$\scriptstyle #1$}}
  \end{picture} }

\def\pupl#1{
  \begin{picture}(8,20)
  \put (4,-10){\vector(0,1){30}}
  \put (1,6){\makebox(1,1)[r]{$\scriptstyle #1$}}
  \end{picture} }

\def\pupr#1{
  \begin{picture}(8,20)
  \put (4,-10){\vector(0,1){30}}
  \put (7,6){\makebox(1,1)[l]{$\scriptstyle #1$}}
  \end{picture} }

\def\pust{
  \begin{picture}(20,20)
  \put (0,0){\makebox(20,20)}
  \end{picture} }

\def\Ra#1{\mathop{\Rightarrow}\limits^{#1}}

\def\ra#1{\mathop{\to}\limits^{#1}}

\def\raa#1#2{\mathop{\to}\limits^{#1}_{#2}}

\def\la#1#2{\mathop{#1}\limits_{#2}}

\def\rea#1{\mbox{$\mathop{\to}\!\!\!\!\!\!\mathop{\to}\limits^{#1}$}}

\def\rog#1#2#3{               \begin{picture}(20,20)
  \put (12,21){\vector(1,-3){19}}
  \put (15,-7){\makebox(1,1)[r]{$\scriptstyle #1$}}
  \multiput (16,23)(3,-3){4}{\vector(1,-1){2}}
  \put(28,11){\vector(1,-1){3}}
  \put (23,17){\makebox(1,1)[l]{$\scriptstyle #2$}}
  \put (18,26){\vector(3,-1){58}}
  \put (50,19){\makebox(1,1)[l]{$\scriptstyle #3$}}
  \end{picture} } 

\def\rogo#1#2{
  \begin{picture}(20,20)
  \put (12,21){\vector(1,-3){19}}
  \put (15,-7){\makebox(1,1)[r]{$\scriptstyle #1$}}
  \put (18,26){\vector(3,-1){58}}
  \put (50,19){\makebox(1,1)[l]{$\scriptstyle #2$}}
  \end{picture} } 

\def\rma#1{\mathop{\hookrightarrow}\limits^{#1}}

\def\tils#1{\mathop{\sim}\limits_{#1}}

\def\tr{{\bf Trnkov\'a V.}}

\def\treug#1#2{
  \begin{picture}(20,20)
  \put (-8,25){\vector(2,-1){30}}
  \put (0,15){ \makebox(15,13)[l]{$\scriptstyle #1$}}
  \put (22,0){\vector(-2,-1){30}}
  \put (7,-14){ \makebox(17,8)[l]{$\scriptstyle #2$}}
  \end{picture} }

\def\treugleft#1#2{
  \begin{picture}(20,20)
  \put (-6,8){\vector(2,1){30}}
  \put (5,18){ \makebox(1,1)[r]{$\scriptstyle #1$}}
  \put (-6,-2){\vector(2,-1){30}}
  \put (5,-17){ \makebox(1,1)[r]{$\scriptstyle #2$}}
  \end{picture} }

\def\treugright#1#2{
  \begin{picture}(20,20)
  \put (-7,23){\vector(2,-1){30}}
  \put (3,20){ \makebox(1,1)[l]{$\scriptstyle #1$}}
  \put (-7,-17){\vector(2,1){30}}
  \put (5,-16){ \makebox(1,1)[l]{$\scriptstyle #2$}}
  \end{picture}}

\def\vright#1{
  \begin{picture}(20,8)
  \put (-15,3){\vector(1,0){50}}
  \put (9,8){\makebox(1,1){$\scriptstyle #1$}}
  \end{picture} }

\def\vsearl#1{
  \begin{picture}(20,20)
  \put (-20,20){\vector(2,-1){60}}
  \put (1,2){ \makebox(1,1)[r]{$\scriptstyle #1$}}
  \end{picture} }

\def\vsearr#1{
  \begin{picture}(20,20)
  \put (-20,20){\vector(2,-1){60}}
  \put (15,9){ \makebox(1,1)[r]{$\scriptstyle #1$}}
  \end{picture} }

\def\vvsearl#1{
  \begin{picture}(20,20)
  \put (-20,20){\vector(2,-1){70}}
  \put (1,2){ \makebox(1,1)[r]{$\scriptstyle #1$}}
  \end{picture} }


%========================================================================



\def\cla{${\cal C}_{(d,f)}\;$}
\def\fuup#1#2{\mathop{#1}\limits^{#2}}
\def\ms#1#2{\{#1\;\vert\;#2\}}
\def\SKIP{\leftskip=-0.6cm
\rightskip=0.6cm}
\def\rog#1#2#3{
  \begin{picture}(20,20)
  \put (12,21){\vector(1,-3){19}}
  \put (15,-7){\makebox(1,1)[r]{$\scriptstyle #1$}}
  \put(16,23){\vector(1,-1){15}}
  \put (23,17){\makebox(1,1)[l]{$\scriptstyle #2$}}
  \put (18,26){\vector(3,-1){58}}
  \put (50,19){\makebox(1,1)[l]{$\scriptstyle #3$}}
  \end{picture} }  

\def\pmonorightlong#1{
  \begin{picture}(20,8)
  \put (-9,2){\vector(1,0){41}}
  \put (-9,4){\oval(4,4)[l]}
  \put (-9,6){\line(1,0){2}}
  \put (11,6){\makebox(1,1){$\scriptstyle #1$}}
  \end{picture} }

\def\eqo{
\mathop{\sim}\limits^o}

\def\cirsc{{\scriptscriptstyle\circ}}

\def\pmonoright#1{
  \begin{picture}(20,8)
  \put (-4,2){\vector(1,0){31}}
  \put (-4,4){\oval(4,4)[l]}
  \put (-4,6){\line(1,0){2}}
  \put (11,6){\makebox(1,1){$\scriptstyle #1$}}
  \end{picture} }

\def\bcoam#1#2#3#4{
  \begin{picture}(20,20)
  \put (15,23){\vector(1,-3){20}}
  \put (15,-5){ \makebox(1,1)[r]{$\scriptstyle #1$}}

  \put (20,25){\vector(1,-1){15}}
  \put (27,19){\makebox(1,1)[l]{$\scriptstyle #2$}}
  \put (83,23){\vector(1,-3){20}}
  \put (85,-5){ \makebox(1,1)[r]{$\scriptstyle #4$}}
  \put (90,23){\vector(1,-1){15}}
  \put (95,18){ \makebox(1,1)[l]{$\scriptstyle #3$}}
  \end{picture} } 

\def\psearl#1{
  \begin{picture}(20,20)
  \put (-5,20){\vector(1,-1){30}}
  \put (1,2){ \makebox(1,1)[r]{$\scriptstyle #1$}}
  \end{picture} } 

\def\psearr#1{
  \begin{picture}(20,20)
  \put (-5,20){\vector(1,-1){30}}
    \put (10,8){\makebox(1,1)[l]{$\scriptstyle #1$}}
  \end{picture} } 

\def\pswarl#1{
  \begin{picture}(20,20)
  \put (25,20){\vector(-1,-1){30}}
  \put (9,8){\makebox(1,1)[r]{$\scriptstyle #1$}}
  \end{picture} } 

\def\pswarr#1{
  \begin{picture}(20,20)
  \put (25,20){\vector(-1,-1){30}}
  \put (14,4){\makebox(1,1)[l]{$\scriptstyle #1$}}
  \end{picture} } 

\def\pright#1{
  \begin{picture}(20,8)
  \put (-5,3){\vector(1,0){30}}
  \put (9,7){\makebox(1,1){$\scriptstyle #1$}}
  \end{picture} }

\def\pdownl#1{
  \begin{picture}(8,20)
  \put (4,20){\vector(0,-1){28}}
  \put (1,6){\makebox(1,1)[r]{$\scriptstyle #1$}}
  \end{picture} }
  
\def\pdownr#1{
  \begin{picture}(8,20)
  \put (4,20){\vector(0,-1){28}}
  \put (7,6){\makebox(1,1)[l]{$\scriptstyle #1$}}
  \end{picture} }

%dash

\def\pdashmonoright#1{
  \begin{picture}(20,8)
  \multiput(-4,2)(5,0){5}{\line(1,0){3}}
  \put (21,2){\vector(1,0){5}}
  \put (-4,4){\oval(4,4)[l]}
  \put (-4,6){\line(1,0){2}}
  \put (11,6){\makebox(1,1){$\scriptstyle #1$}}
  \end{picture} }

\def\pdashright#1{
  \begin{picture}(20,8)
  \multiput (-5,3)(5,0){5}{\line(1,0){3}}
  \put (20,3){\vector(1,0){5}}
  \put (9,7){\makebox(1,1){$\scriptstyle #1$}}
  \end{picture} }

\def\pdashdownl#1{
  \begin{picture}(8,20)
  \multiput (4,20)(0,-5){5}{\line(0,-1){3}}
  \put(4,-5){\vector(0,-1){3}}
  \put (1,6){\makebox(1,1)[r]{$\scriptstyle #1$}}
  \end{picture} }
  
\def\pdashdownr#1{
  \begin{picture}(8,20)
  \multiput (4,20)(0,-5){5}{\line(0,-1){3}}
  \put(4,-5){\vector(0,-1){3}}
  \put (7,6){\makebox(1,1)[l]{$\scriptstyle #1$}}
  \end{picture} }
  
%end dash  
  
\def\mironov#1{
\begin{picture}(20,20)
\put (-5,3){\line(1,0){45}}
\put (40,-7){\oval(20,20)[tr]}
\put (50,-7){\line(0,-1){68}}
\put (40,-75){\oval(20,20)[br]}
\put (40,-85){\vector(-1,0){45}}
\put (52,-40){\makebox (16,8){$\scriptstyle #1$}}
\end{picture} }

\def\psesp#1{
  \begin{picture}(20,20)
  \put (15,20){\vector(2,-3){50}}
  \put (10,-25){ \makebox(22,8)[r]{$\scriptstyle #1$}}
  \end{picture} } 

\def\pust{
  \begin{picture}(20,20)
  \put (0,0){\makebox(20,20)}
  \end{picture} }

\def\treug#1#2{
  \begin{picture}(20,20)
  \put (-8,25){\vector(2,-1){30}}
  \put (0,15){ \makebox(15,13)[l]{$\scriptstyle #1$}}
  \put (22,0){\vector(-2,-1){30}}
  \put (7,-14){ \makebox(17,8)[l]{$\scriptstyle #2$}}
  \end{picture} }

\def\eqd{\buildrel \rm def \over\Longleftrightarrow}
\def\eam{\buildrel \rm def \over =}
\def\os{\mbox{$\Omega$-$Set$ }}
\def\a#1{\mbox{$#1$}}
\def\db#1#2#3{[\![{#1},{#2}]\!]_{#3}}
\def\hs#1{$(#1;[\![,]\!]_{#1})$}
\def\op#1#2{\langle{#1},{#2}\rangle}
\def\bcd#1{
  \begin{picture}(20,20)
   \put(10,10){\circle{20}} 
   \put(10,10){\mbox{#1}}    
  \end{picture} }
  

\def\a#1{\mbox{$#1$}}

\def\ad{{\bf Ad\'amek J.}}

\def\bcd#1{
  \begin{picture}(20,20)
   \put(10,10){\circle{20}}
   \put(10,10){\mbox{#1}}
  \end{picture} }

\def\bcoam#1#2#3#4{
  \begin{picture}(20,20)
  \put (15,23){\vector(1,-3){20}}
  \put (15,-5){ \makebox(1,1)[r]{$\scriptstyle #1$}}
  \multiput (20,25)(3,-3){4}{\vector(1,-1){2}}
  \put(32,13){\vector(1,-1){3}}
  \put (27,19){\makebox(1,1)[l]{$\scriptstyle #2$}}
  \put (83,23){\vector(1,-3){20}}
  \put (85,-5){ \makebox(1,1)[r]{$\scriptstyle #4$}}
  \put (90,23){\vector(1,-1){15}}
  \put (95,18){ \makebox(1,1)[l]{$\scriptstyle #3$}}
  \end{picture} } 

\def\ci#1{$(#1)$ }

\def\cii#1{$(#1)$}

\def\cirsc{{\scriptscriptstyle\circ}}

\def\ciz#1{$(#1)$}

\def\corog#1#2#3{             \begin{picture}(20,20)
  \put (-35,23){\vector(3,-1){60}}
  \put (-8,8){\makebox(1,1)[r]{$\scriptstyle #1$}}
  \multiput (14,21)(3,-3){4}{\vector(1,-1){2}}
  \put (26,9){\vector(1,-1){3}}
  \put (22,17){\makebox(1,1)[l]{$\scriptstyle #2$}}
  \put (14,65){\vector(1,-3){19}}
  \put (24,40){\makebox(1,1)[l]{$\scriptstyle #3$}}
\end{picture} }
  
\def\db#1#2#3{[\![{#1},{#2}]\!]_{#3}}

\def\dpright#1#2{    \begin{picture}(20,8)
    \put (-5,4){\vector(1,0){30}}
    \put (9,8){\makebox(1,1){$\scriptstyle #1$}}
    \put (-5,1){\vector(1,0){30}}
    \put (9,-3){\makebox(1,1){$\scriptstyle #2$}}
    \end{picture} }

\def\eam{\buildrel \rm def \over =}

\def\ep{\;\mbox{$\mathop{\to}{\!\!\!\!\!.}$}\;}

\def\epi{\mbox{$\mathop{\to}\!\!\!\!\!\!\mathop{\to}$}}

\def\eqd{\buildrel \rm def \over\Longleftrightarrow}

\def\eqo{\mathop{\sim}\limits^o}

\def\exp#1#2#3#4{
\diagr{#3&\!\!\!\!\times\!\!\!\!&#1\cr
\pdashdownl{\hat{#4}}&\!\!\!\!
\begin{picture}(1,10)
\put (-3,3){\mbox{$\mathop{\times}$}}
\end{picture}\!\!\!\!
&\pdownr{id_#1}&\psearr{#4}\cr
#2^#1&\!\!\!\!\times\!\!\!\!&#1&\prightd{ev_{#1,#2}}&#2\cr
}}

\def\fd{${\cal F}_{{\cal F},D}$}

\def\fuup#1#2{\mathop{#1}\limits^{#2}}

\def\goa{\mbox{$\Gamma$-$\Omega$-$Alg$ }}

\def\gs{\mbox{$\Gamma$-$Set$ }}

\def\hs#1{$(#1;[\![,]\!]_{#1})$}



\def\md{{\cal M}_D}

\def\mdn#1{{\cal M}_{D_#1}}

\def\mil#1{
\begin{picture}(20,20)
\put (30,3){\line(-1,0){5}}
\put (25,-7){\oval(20,20)[tl]}
\put (15,-7){\line(0,-1){71}}
\put (25,-78){\oval(20,20)[bl]}
\put (25,-88){\vector(1,0){5}}
\put (-2,-45){\makebox (16,8)[r]{$\scriptstyle #1$}}
\end{picture} }

\def\milcc#1{
\begin{picture}(20,20)
\put (33,3){\line(-1,0){2}}
\put (31,1){\oval(4,4)[tl]}
\put (29,1){\line(0,-1){74}}
\put (29,-73){\vector(1,-1){10}}
\put (9,-23){\makebox (16,8)[r]{$\scriptstyle #1$}}
\end{picture}}

\def\milongl#1{
\begin{picture}(20,20)
\put (30,3){\line(-1,0){5}}
\put (25,-7){\oval(20,20)[tl]}
\put (15,-7){\line(0,-1){115}}
\put (25,-122){\oval(20,20)[bl]}
\put (25,-132){\vector(1,0){5}}
\put (-2,-67){\makebox (16,8)[r]{$\scriptstyle #1$}}
\end{picture} }

\def\milongr#1{
\begin{picture}(20,20)
\put (-10,3){\line(1,0){5}}
\put (-5,-7){\oval(20,20)[tr]}
\put (5,-7){\line(0,-1){115}}
\put (-5,-122){\oval(20,20)[br]}
\put (-5,-132){\vector(-1,0){5}}
\put (8,-67){\makebox (16,8)[l]{$\scriptstyle #1$}}
\end{picture} }

\def\mir#1{
\begin{picture}(20,20)
\put (-10,3){\line(1,0){5}}
\put (-5,-7){\oval(20,20)[tr]}
\put (5,-7){\line(0,-1){71}}
\put (-5,-78){\oval(20,20)[br]}
\put (-5,-88){\vector(-1,0){5}}
\put (8,-45){\makebox (16,8)[l]{$\scriptstyle #1$}}
\end{picture} }

\def\mircc#1{
\begin{picture}(20,20)
\put (-10,3){\line(1,0){2}}
\put (-8,1){\oval(4,4)[tr]}
\put (-6,1){\line(0,-1){74}}
\put (-6,-73){\vector(-1,-1){10}}
\put (-10,-23){\makebox (1,8)[r]{$\scriptstyle #1$}}
\end{picture} }

\def\mironov#1{
\begin{picture}(20,20)
\put (-5,3){\line(1,0){45}}
\put (40,-7){\oval(20,20)[tr]}
\put (50,-7){\line(0,-1){68}}
\put (40,-75){\oval(20,20)[br]}
\put (40,-85){\vector(-1,0){45}}
\put (52,-40){\makebox (16,8){$\scriptstyle #1$}}
\end{picture} }

\def\mit#1{
\begin{picture}(20,20)
\put (10,-10){\line(0,1){5}}
\put (20,-5){\oval(20,20)[tl]}
\put (20,5){\line(1,0){100}}
\put (120,-5){\oval(20,20)[tr]}
\put (130,-5){\vector(0,-1){5}}
\put (-45,-2){\makebox (16,8)[r]{$\scriptstyle #1$}}
\end{picture} }

\def\mitblong#1{
\begin{picture}(20,20)
\put (10,15){\line(0,1){5}}
\put (20,15){\oval(20,20)[bl]}
\put (20,5){\line(1,0){225}}
\put (245,15){\oval(20,20)[br]}
\put (255,15){\vector(0,1){5}}
\put (138,10){\makebox (1,1)[c]{$\scriptstyle #1$}}
\end{picture} }

\def\mittlong#1{
\begin{picture}(20,20)
\put (10,-10){\line(0,1){5}}
\put (20,-5){\oval(20,20)[tl]}
\put (20,5){\line(1,0){225}}
\put (245,-5){\oval(20,20)[tr]}
\put (255,-5){\vector(0,-1){5}}
\put (138,10){\makebox (1,1)[c]{$\scriptstyle #1$}}
\end{picture} }

\def\ms#1#2{\{#1\;\vert\;#2\}}

\def\oa{\mbox{$\Omega$-$Alg$ }}

\def\op#1#2{\langle{#1},{#2}\rangle}

\def\os{\mbox{$\Omega$-$Set$ }}

\def\pairarr#1#2{
\begin{picture}(10,10)
\put (0,6){$\mathop{\longrightarrow}$}
\put (6,11){\framebox(1,1){$\scriptstyle #1$}}
\put (0,4){$\mathop{\longleftarrow}$}
\put (6,2) {\framebox(1,1){$\scriptstyle #2$}}
\end{picture}}

\def\pbigbigright#1{
  \begin{picture}(50,8)
  \put (-15,3){\vector(1,0){80}}
  \put (24,8){\makebox(1,1){$\scriptstyle #1$}}
  \end{picture}}

\def\pbigdashright#1{
  \begin{picture}(50,8)
  \multiput (-20,3)(5,0){16}{\line(1,0){3}}
  \put (60,3){\vector(1,0){5}}
  \put (20,7){\makebox(1,1){$\scriptstyle #1$}}
  \end{picture} }

\def\pbigright#1{
\begin{picture}(50,8)
  \put (-5,3){\vector(1,0){60}}
  \put (24,8){\makebox(1,1){$\scriptstyle #1$}}
  \end{picture}}

\def\pdashdownl#1{
  \begin{picture}(8,20)
  \multiput (4,20)(0,-5){5}{\line(0,-1){3}}
  \put(4,-5){\vector(0,-1){5}}
  \put (1,6){\makebox(1,1)[r]{$\scriptstyle #1$}}
  \end{picture} }

\def\pdashdownr#1{
  \begin{picture}(8,20)
  \multiput (4,20)(0,-5){5}{\line(0,-1){3}}
  \put(4,-5){\vector(0,-1){5}}
  \put (7,6){\makebox(1,1)[l]{$\scriptstyle #1$}}
  \end{picture} }

\def\pdashmonoright#1{
  \begin{picture}(20,8)
  \multiput(-4,2)(5,0){5}{\line(1,0){3}}
  \put (21,2){\vector(1,0){5}}
  \put (-4,4){\oval(4,4)[l]}
  \put (-4,6){\line(1,0){2}}
  \put (11,6){\makebox(1,1){$\scriptstyle #1$}}
  \end{picture} }

\def\pdashright#1{
  \begin{picture}(20,8)
  \multiput (-5,3)(5,0){5}{\line(1,0){3}}
  \put (20,3){\vector(1,0){5}}
  \put (9,7){\makebox(1,1){$\scriptstyle #1$}}
  \end{picture} }

\def\pdashsearl#1{
  \begin{picture}(20,20)
  \put (-5,20){\line (1,-1){10}}
  \put (7,8){\line (1,-1){10}}
  \put (19,-4){\vector(1,-1){10}}
  \put (-20,0){ \makebox(1,1)[r]{$\scriptstyle #1$}}
  \end{picture} }

\def\pdashsearr#1{
  \begin{picture}(20,20)
  \put (-5,20){\vector(1,-1){30}}
    \put (12,5){\makebox(1,1)[l]{$\scriptstyle #1$}}
  \end{picture} }

\def\pdashswarl#1{
  \begin{picture}(20,20)
  \put (25,20){\vector(-1,-1){30}}
  \put (-15,5){\makebox(1,1)[r]{$\scriptstyle #1$}}
  \end{picture} }

\def\pdashswarr#1{
  \begin{picture}(20,20)
  \put (25,20){\vector(-1,-1){30}}
  \put (17,0){\makebox(1,1)[l]{$\scriptstyle #1$}}
  \end{picture} }

\def\pdoubledown#1#2{
\begin{picture}(8,20)
  \put (1,20){\vector(0,-1){30}}
  \put (-2,6){\makebox(1,1)[r]{$\scriptstyle #1$}}
  \put (5,20){\vector(0,-1){30}}
  \put (8,6){\makebox(1,1)[l]{$\scriptstyle #2$}}
  \end{picture}}

\def\pdownl#1{
  \begin{picture}(8,20)
  \put (4,20){\vector(0,-1){28}}
  \put (1,6){\makebox(1,1)[r]{$\scriptstyle #1$}}
  \end{picture} }

\def\pdownlongl#1{
  \begin{picture}(8,20)
  \put (4,20){\vector(0,-1){75}}
  \put (1,-16){\makebox(1,1)[r]{$\scriptstyle #1$}}
  \end{picture} }

\def\pdownlongr#1{
  \begin{picture}(8,20)
  \put (4,20){\vector(0,-1){75}}
  \put (7,-16){\makebox(1,1)[l]{$\scriptstyle #1$}}
  \end{picture} }

\def\pdownr#1{
  \begin{picture}(8,20)
  \put (4,20){\vector(0,-1){28}}
  \put (7,6){\makebox(1,1)[l]{$\scriptstyle #1$}}
  \end{picture} }

\def\pepidownl#1{
  \begin{picture}(8,20)
  \put (4,20){\vector(0,-1){30}}
  \put (4,-3){\vector(0,-1){5}}
  \put (1,6){\makebox(1,1)[r]{$\scriptstyle #1$}}
  \end{picture} }
  
\def\pepidownr#1{
  \begin{picture}(8,20)
  \put (4,20){\vector(0,-1){30}}
  \put (4,-3){\vector(0,-1){5}}
  \put (7,6){\makebox(1,1)[l]{$\scriptstyle #1$}}
  \end{picture} }

\def\pepiright#1{
  \begin{picture}(20,8)
  \put (-5,3){\vector(1,0){30}}
  \put (18,3){\vector(1,0){5}}
  \put (9,7){\makebox(1,1){$\scriptstyle #1$}}
  \end{picture} }

\def\pleftdouble#1#2
{
\begin{picture}(20,8)
  \put (25,5){\vector(-1,0){30}}
  \put (11,9){\makebox(1,1){$\scriptstyle {#1}$}}
  \put (25,1){\vector(-1,0){30}}
  \put (11,-3){\makebox(1,1){$\scriptstyle {#2}$}}
  \end{picture}
}

\def\plongright#1{
  \begin{picture}(20,8)
  \put (-5,3){\vector(1,0){115}}
  \put (50,8){\makebox(1,1){$\scriptstyle #1$}}
  \end{picture} }

\def\pmiddleright#1{
  \begin{picture}(35,8)
  \put (-5,3){\vector(1,0){45}}
  \put (17,8){\makebox(1,1){$\scriptstyle #1$}}
  \end{picture} }

\def\pmonodownl#1{
  \begin{picture}(8,20)
  \put (4,18){\vector(0,-1){28}}
  \put (6,18){\oval(4,4)[t]}
  \put (8,18){\line(0,-1){2}}
  \put (1,6){\makebox(1,1)[r]{$\scriptstyle #1$}}
  \end{picture} }
  
\def\pmonodownr#1{
  \begin{picture}(8,20)
  \put (4,18){\vector(0,-1){28}}
  \put (2,18){\oval(4,4)[t]}
  \put (0,18){\line(0,-1){2}}
  \put (7,6){\makebox(1,1)[l]{$\scriptstyle #1$}}
  \end{picture} }

\def\pmonoright#1{
  \begin{picture}(20,8)
  \put (-4,2){\vector(1,0){31}}
  \put (-4,4){\oval(4,4)[l]}
  \put (-4,6){\line(1,0){2}}
  \put (11,6){\makebox(1,1){$\scriptstyle #1$}}
  \end{picture} }

\def\pmonorightlong#1{
  \begin{picture}(20,8)
  \put (-9,2){\vector(1,0){41}}
  \put (-9,4){\oval(4,4)[l]}
  \put (-9,6){\line(1,0){2}}
  \put (11,6){\makebox(1,1){$\scriptstyle #1$}}
  \end{picture} }

\def\pnearr#1{
  \begin{picture}(20,20)
  \put (-5,-10){\vector(1,1){30}}
  \put (10,5){ \makebox(1,1)[l]{$\scriptstyle #1$}}
  \end{picture} }

\def\pneearr#1{
\begin{picture}(20,20)
  \put (0,0){\vector(3,2){40}}
  \put (1,2){ \makebox(1,1)[r]{$\scriptstyle #1$}}
  \end{picture}
}

\def\pnnearr#1{
  \begin{picture}(20,20)
  \put (-11,-10){\vector(1,2){38}}
  \put (10,28){ \makebox(1,1)[l]{$\scriptstyle #1$}}
  \end{picture} }

\def\pright#1{
  \begin{picture}(20,8)
  \put (-5,3){\vector(1,0){30}}
  \put (9,8){\makebox(1,1){$\scriptstyle #1$}}
  \end{picture} }

\def\prightd#1{
  \begin{picture}(20,8)
  \put (-5,3){\vector(1,0){30}}
  \put (9,-2){\makebox(1,1){$\scriptstyle #1$}}
  \end{picture} }

\def\prightdouble#1#2
{
\begin{picture}(20,8)
  \put (-5,5){\vector(1,0){30}}
  \put (11,10){\makebox(1,1){$\scriptstyle {#1}$}}
  \put (-5,1){\vector(1,0){30}}
  \put (11,-5){\makebox(1,1){$\scriptstyle {#2}$}}
  \end{picture}
}

\def\prightlong#1{
  \begin{picture}(20,8)
  \put (-5,3){\vector(1,0){35}}
  \put (11,7){\makebox(1,1){$\scriptstyle #1$}}
  \end{picture} }

\def\prightmiddle#1{
  \begin{picture}(20,8)
  \put (-10,3){\vector(1,0){40}}
  \put (9,8){\makebox(1,1){$\scriptstyle #1$}}
  \end{picture} }

\def\prightright#1{
  \begin{picture}(20,8)
  \put (-5,3){\vector(1,0){40}}
  \put (14,8){\makebox(1,1){$\scriptstyle #1$}}
  \end{picture} }

\def\prightsuperlong#1{
  \begin{picture}(20,8)
  \put (-5,3){\vector(1,0){49}}
  \put (18,7){\makebox(1,1){$\scriptstyle #1$}}
  \end{picture} }

\def\pseardouble#1{
  \begin{picture}(20,20)
  \put (-5,20){\vector(1,-1){30}}
  \put (-8,17){\vector(1,-1){30}}
  \put (1,2){ \makebox(1,1)[r]{$\scriptstyle #1$}}
  \end{picture} }

\def\psearl#1{
  \begin{picture}(20,20)
  \put (-5,20){\vector(1,-1){30}}
  \put (4,2){ \makebox(1,1)[r]{$\scriptstyle #1$}}
  \end{picture} }

\def\psearlongl#1{
  \begin{picture}(20,20)
  \put (-5,20){\vector(3,-1){105}}
  \put (41,-1){ \makebox(1,1)[r]{$\scriptstyle #1$}}
  \end{picture}}

\def\psearr#1{
  \begin{picture}(20,20)
  \put (-5,20){\vector(1,-1){30}}
    \put (10,8){\makebox(1,1)[l]{$\scriptstyle #1$}}
  \end{picture} }

\def\pseearl#1{
  \begin{picture}(20,20)
  \put (-20,40){\vector(3,-1){100}}
  \put (1,2){ \makebox(1,1)[r]{$\scriptstyle #1$}}
  \end{picture} }

\def\pseearr#1{
\begin{picture}(20,20)
  \put (-5,0){\vector(3,-2){40}}
  \put (1,2){ \makebox(1,1)[r]{$\scriptstyle #1$}}
  \end{picture}
}

\def\psesp#1{
  \begin{picture}(20,20)
  \put (15,20){\vector(2,-3){50}}
  \put (10,-25){ \makebox(22,8)[r]{$\scriptstyle #1$}}
  \end{picture} }

\def\psseardashr#1{
 \begin{picture}(20,20)
  \multiput(-5,20)(5,-10){5}{\line(1,-2){4}}
  \put (20,-30){\vector(1,-2){5}}
  \put (1,2){ \makebox(1,1)[r]{$\scriptstyle #1$}}
  \end{picture} }

\def\psseardouble#1#2{
  \begin{picture}(20,20)
  \put (-18,18){\vector(1,-1){70}}
  \put (-21,15){\vector(1,-1){70}}
  \put (3,-19){ \makebox(1,1)[r]{$\scriptstyle #1$}}
  \put (15,-13){ \makebox(1,1)[l]{$\scriptstyle #2$}}
  \end{picture} }

\def\pssearr#1
{
\begin{picture}(20,20)
  \put (-8,20){\vector(1,-2){37}}
  \put (10,-10){\makebox(1,1)[l]{$\scriptstyle {#1}$}}
\end{picture}
}

\def\pswarl#1{
  \begin{picture}(20,20)
  \put (25,20){\vector(-1,-1){30}}
  \put (9,8){\makebox(1,1)[r]{$\scriptstyle #1$}}
  \end{picture} }

\def\pswarr#1{
  \begin{picture}(20,20)
  \put (25,20){\vector(-1,-1){30}}
  \put (14,4){\makebox(1,1)[l]{$\scriptstyle #1$}}
  \end{picture} }

\def\pupl#1{
  \begin{picture}(8,20)
  \put (4,-10){\vector(0,1){30}}
  \put (1,6){\makebox(1,1)[r]{$\scriptstyle #1$}}
  \end{picture} }

\def\pupr#1{
  \begin{picture}(8,20)
  \put (4,-10){\vector(0,1){30}}
  \put (7,6){\makebox(1,1)[l]{$\scriptstyle #1$}}
  \end{picture} }

\def\pust{
  \begin{picture}(20,20)
  \put (0,0){\makebox(20,20)}
  \end{picture} }

\def\ra#1{\mathop{\to}\limits^{#1}}

\def\rea#1{\mbox{$\mathop{\to}\!\!\!\!\!\!\mathop{\to}\limits^{#1}$}}

\def\rog#1#2#3{               \begin{picture}(20,20)
  \put (12,21){\vector(1,-3){19}}
  \put (15,-7){\makebox(1,1)[r]{$\scriptstyle #1$}}
%  \multiput (16,23)(3,-3){4}{\line(1,-1){2}}
  \put(16,23){\vector(1,-1){15}}
  \put (23,17){\makebox(1,1)[l]{$\scriptstyle #2$}}
  \put (18,26){\vector(3,-1){58}}
  \put (50,19){\makebox(1,1)[l]{$\scriptstyle #3$}}
  \end{picture} } 

\def\rogo#1#2{
  \begin{picture}(20,20)
  \put (12,21){\vector(1,-3){19}}
  \put (15,-7){\makebox(1,1)[r]{$\scriptstyle #1$}}
  \put (18,26){\vector(3,-1){58}}
  \put (50,19){\makebox(1,1)[l]{$\scriptstyle #2$}}
  \end{picture} } 

\def\rma#1{\mathop{\hookrightarrow}\limits^{#1}}

\def\tr{{\bf Trnkov\'a V.}}

\def\treug#1#2{
  \begin{picture}(20,20)
  \put (-8,25){\vector(2,-1){30}}
  \put (0,15){ \makebox(15,13)[l]{$\scriptstyle #1$}}
  \put (22,0){\vector(-2,-1){30}}
  \put (7,-14){ \makebox(17,8)[l]{$\scriptstyle #2$}}
  \end{picture} }

\def\treugleft#1#2{
  \begin{picture}(20,20)
  \put (-6,8){\vector(2,1){30}}
  \put (5,18){ \makebox(1,1)[r]{$\scriptstyle #1$}}
  \put (-6,-2){\vector(2,-1){30}}
  \put (5,-17){ \makebox(1,1)[r]{$\scriptstyle #2$}}
  \end{picture} }

\def\treugright#1#2{
  \begin{picture}(20,20)
  \put (-7,23){\vector(2,-1){30}}
  \put (3,20){ \makebox(1,1)[l]{$\scriptstyle #1$}}
  \put (-7,-17){\vector(2,1){30}}
  \put (5,-16){ \makebox(1,1)[l]{$\scriptstyle #2$}}
  \end{picture}}

\def\vright#1{
  \begin{picture}(20,8)
  \put (-15,3){\vector(1,0){50}}
  \put (9,8){\makebox(1,1){$\scriptstyle #1$}}
  \end{picture} }

\def\vsearl#1{
  \begin{picture}(20,20)
  \put (-20,20){\vector(2,-1){60}}
  \put (1,2){ \makebox(1,1)[r]{$\scriptstyle #1$}}
  \end{picture} }

\def\vsearr#1{
  \begin{picture}(20,20)
  \put (-20,20){\vector(2,-1){60}}
  \put (15,9){ \makebox(1,1)[r]{$\scriptstyle #1$}}
  \end{picture} }

\def\vvsearl#1{
  \begin{picture}(20,20)
  \put (-20,20){\vector(2,-1){70}}
  \put (1,2){ \makebox(1,1)[r]{$\scriptstyle #1$}}
  \end{picture} }


